Peeking with PEAK: Sequential, Nonparametric Composite Hypothesis Tests for Means of Multiple Data Streams

We propose a novel nonparametric sequential test for composite hypotheses for means of multiple data streams. Our proposed method, \emph{peeking with expectation-based averaged capital} (PEAK), builds upon the testing-by-betting framework and provides a non-asymptotic $\alpha$-level test across any stopping time. Our contributions are two-fold: (1) we propose a novel betting scheme and provide theoretical guarantees on type-I error control, power, and asymptotic growth rate/$e$-power in the setting of a single data stream; (2) we introduce PEAK, a generalization of this betting scheme to multiple streams, that (i) avoids using wasteful union bounds via averaging, (ii) is a test of power one under mild regularity conditions on the sampling scheme of the streams, and (iii) reduces computational overhead when applying the testing-as-betting approaches for pure-exploration bandit problems. We illustrate the practical benefits of PEAK using both synthetic and real-world HeartSteps datasets. Our experiments show that PEAK provides up to an 85\% reduction in the number of samples before stopping compared to existing stopping rules for pure-exploration bandit problems, and matches the performance of state-of-the-art sequential tests while improving upon computational complexity.

==> discussion.tex <==
%Empirical and theoretical extensions to our work would include:
%1) tuning the density bound $c$ and convergence tolerance $\gamma, l(\cdot, \cdot)$ for preserving this method's theoretical guarantees,
%2) testing integral approximations in computation of kernel functions $K_0(\cdot, \cdot)$;
In this paper, we introduce KDPE, a new method for debiasing plug-in estimators that (i) does not require the IF as input, (ii) works as a general plug-in for any target parameters that satisfy our regularity conditions. Distinct from existing computational methods that aim to do IF-free debiasing, our approach does \emph{not} make any explicit attempt to approximate the IF, and retains the simplicity of a plug-in approach. 

Future work includes
(i) analyzing the effect of RKHS-norm regularization on the convergence and efficiency, (ii) finding simple heuristics for setting hyperparameters $c, \gamma, \lambda$, 
(iii) investigating how to apply sample-splitting and the extent to which it can relax our assumptions,
(iv) providing primitive conditions for RKHS approximation of the IF score equation (Assumption \ref{assump:S5}), and (v) verifying the validity of bootstrap.
% remains a key question, as well as 
Alternative methods for constructing confidence intervals include directly taking the quantiles of the bootstrap estimates and/or subsampling while bootstrapping, which we do not explore in Appendix \ref{app:simulation}.  The strong connection between our method and TMLE raises the question of whether TMLE variants, such as CTMLE \citep{coyle2023}, CV-TMLE \citep{book2011}, and one-step TMLE \citep{one_step_tmle}, can be adapted to KDPE to reduce computational costs. The empirical performance of KDPE for DGP2 also suggests that KDPE may provide better finite-sample performance. Understanding KDPE's effect on the behavior of the empirical process and second-order remainder terms are directions for future 
% theoretical
work.


==> notation.tex <==
%\red{Under construction}
%\brian{I think for the most part, this is done}
%kyra: great
% I have more to add :)

\begin{description}[
  leftmargin=2.2cm,
  labelwidth=2cm,
  labelsep=.2cm,
  parsep=0mm,
  itemsep=2pt
  ]

\item[${[}n{]}$] set of integers $1,\ldots, n$

\item[$\calO$] Sample space, with $\calO\subset\mR^d$ and Borel $\s$-algebra $\calB$;

\item[$\calM$] Statistical model, collection of probability measures on $(\calO,\calB)$;

\item[$\psi(P)$] Target parameter functional, mapping from $\Mcal \rightarrow \RR$

\item[$\tilde\psi_P$] Influence function, mapping from $\Ocal \rightarrow \RR$

\item[$Pf, P{[}f{]}$] Expectation functional $Pf = P[f] = \int f \, dP$

\item[$\mP_n, \mP_nf$] Empirical distribution function

\item[$L^2_0(P)$] The set of measurable functions $\{f:\Ocal \rightarrow \RR: Pf = 0 \ , Pf^2 < \infty\}$
    
\item[$P^*$] (Unknown) data generating distribution;

\item[$K, \Hcal_K$] The PSD kernel and associated RKHS with kernel function $K(\cdot, \cdot)$

\item[$k_x$] The function 
  $k_x \coloneqq K(x, \cdot): \Xcal \rightarrow \RR$, for $x$ in support $\Xcal$

\item[$k_\mbf{x}$] Vectorized version of function $k_x$, where $k_\mbf{x}\coloneqq [k_{x_1},...,k_{x_n}]^T$

\item[$K_\mbf{xy}, K_\mbf{x}$] Matrix of values $K_\mbf{x} \coloneqq [K(x_i, x_j)]_{i,j} \in \RR{n\times n}$, $K_{\mbf{xy}} \coloneqq [K(x_i, y_j)]_{ij}\in \RR{n\times m}$

\item[$K_P, \Hcal_P$] The mean-zero kernel (with respect to $P$) and associated RKHS

\item[$\widetilde{\Mcal}_P$] The collection of perturbations $\widetilde{\Mcal}_P\coloneqq\{(1+h)p \ |\ h \in \Hcal_P \text{ such that }(1+h)p > 0\}\cap \Mcal$

\item[$\widetilde{\Mcal}_{P, n}$] The set of $n$-dimensional parametric submodels, defined as follows:
\[\widetilde{\Mcal}_{P, n} \coloneqq\Set[\big]{
    p_{\bm{\a}} \coloneqq p(\bm{\a}) \coloneqq
    (1 + \bm{\a}^\top k_\mbf{O})p
  }{
    \bm{\a}\in\mR^n \text{ such that } p(\bm{\a}) > 0
  } \cap \calM \]

\item[$\widetilde\calM^\ell$] The collection of perturbations $\widetilde\Mcal_{P_n^l}$ corresponding to $\ell$-th iteration's distribution, $P_n^l$

\item[$p(\epsilon|h),\ p_{\epsilon, h}$] 1-dimensional parametric model $(1+\epsilon h)p$

\item[$p(h), p_h$] RKHS-based model $(1+h)p$, where $h \in \Hcal_{P}$

%\item[$\h{p}_n(\alpha, p)$] $n$-dimensional parametric model $(1+\sum_{i=1}^n\alpha_i K_{P}(O_i, \cdot))p(\cdot)$

\item[$L_{p, h}$] Log-likelihood likelihood loss, given by $L_{p,h}\equiv -\log(p_h)$

%\item[$L(p_h, \lambda)$] Regularized log-likelihood objective function $-\frac{1}{n}\sum_{i=1}^n \log(p_h(O_i)) + \lambda\|h\|_{\Hcal_{P_h}}^2$

%\item[$L(\h{p}_n(\alpha, p), \lambda)$] Regularized log-likelihood objective function with $n$-dimensional parametric model: \[L(\h{p}_n(\alpha, p), \lambda)=-\frac{1}{n}\sum_{j=1}^n\Big(
%        \log\Big(\Big(1+\sum_{i=1}^n \a_i K_{P}(O_i, O_j)\Big)p(O_j)\Big) 
%    \Big) 
%    +
%    \lambda\|
%        \sum_{i=1}^n \a_i K_{P}(O_i, \cdot)
%    \|^2_{\calH_{P}}\]

%\item[$L(\h{p}_n(\alpha, p))$] Log-likelihood objective function $L(\h{p}_n(\alpha, p)) \coloneqq L(\h{p}_n(\alpha, p), 0)$ 
\item[$D_P\psi$] Derivative functional (assumed to be continuous, linear) that maps $L_0^2(P)\rightarrow \RR$,\newline $\frac{d}{d\epsilon}\psi({P_{\epsilon, h}})|_{\epsilon=0}=D_P\psi[h]$ for all $h \in L_0^2(P)$

\item[$\pi_S$] The orthogonal projection operator $\Hcal \rightarrow S$, projects a function $h \in \Hcal$ onto a set of functions $S$

\item[$\bm\a_n^i$] The optimal perturbation for objective function $L(\h{p}_n(\alpha, p), \lambda)$ at iteration $i$ for KDPE

\item[$P_n^i, \ p_n^i$] Estimated data distribution of TMLE/KDPE at iteration $i$

\item[$P^\infty_n, \ p_n^\infty$] Limiting/final estimate for TMLE/KDPE

\item[$\h{P}$] Generic estimated distribution, subscripts/superscript added accordingly

\item[$\h\psi_{\text{param.}}$] Estimated target parameter value $\psi_{\text{param.}}(\h P)$ using plug-in distribution $\h P$, subscripts/superscript added accordingly

\item[$Q(P)$] Relevant portion of distribution (e.g. $
\{Q_a(X)\}_{a \in \{0,1\}}= \{P[Y=1|X, A=a]\}_{a\in \{0,1\}}$).

\item[$\Omega$] An event (or set of events) such that has probability 1 under $P^*$, i.e. $P^*(\Omega)=1$. The standard example is the set of all possible $n$-sample realizations $\{\{O_i(w)\}_{i=1}^n \ :\ w \in \Omega\}$ from distribution $P^*$.   

\item[$f(w), P(w)$] The random function / distribution, indexed by events $w \in \Omega$. Often, we use $w \in \Omega$ to index an $n$-sample realization, $\{O_i(w)\}_{i=1}^n$, from DGP $P^*$.   
\end{description}

